Exploring User Opinions of Fairness in Recommender Systems

Algorithmic fairness for artificial intelligence has become increasingly relevant as these systems become more pervasive in society. One realm of AI, recommender systems, presents unique challenges for fairness due to trade offs between optimizing accuracy for users and fairness to providers. But what is fair in the context of recommendation--particularly when there are multiple stakeholders? In an initial exploration of this problem, we ask users what their ideas of fair treatment in recommendation might be, and why. We analyze what might cause discrepancies or changes between user's opinions towards fairness to eventually help inform the design of fairer and more transparent recommendation algorithms.

==> FRA_CHI2020.tex <==
% \begin{document}

%% For the camera ready, use the commands provided by the ACM in the Permission Release Form.

\section{Introduction}
Intro Here


\section{Relevant Work}
Probably something about algorithmic fairness, user folk-theory of algorithms and recsys, recommender fairness, transparency & explanations, and trust.

% \marginpar{%
%   \vspace{-45pt} \fbox{%
%     \begin{minipage}{0.925\marginparwidth}
%       \textbf{Good Utilization of the Side Bar} \\
%       \vspace{1pc} \textbf{Preparation:} Do not change the margin
%       dimensions and do not flow the margin text to the
%       next page. \\
%       \vspace{1pc} \textbf{Materials:} The margin box must not intrude
%       or overflow into the header or the footer, or the gutter space
%       between the margin paragraph and the main left column. The text
%       in this text box should remain the same size as the body
%       text. Use the \texttt{{\textbackslash}vspace{}} command to set
%       the margin
%       note's position. \\
%       \vspace{1pc} \textbf{Images \& Figures:} Practically anything
%       can be put in the margin if it fits. Use the
%       \texttt{{\textbackslash}marginparwidth} constant to set the
%       width of the figure, table, minipage, or whatever you are trying
%       to fit in this skinny space.
%     \end{minipage}}\label{sec:sidebar} }

\section{Methodology?}
Conducted X interviews of Y people, etc..
\section{Interview Analyses}
Human perceptions of algorithmic fairness in for-profit vs non-profit organizations (ie Kiva vs Amazon).
\subsubsection{Sense of Fairness}
Prioritisation of fair and unfair algorithms, ie. do users expect Kiva to be fair? do users expect Amazon to be fair? do users think Kiva/Amazon is fair right now? do users want Kiva/Amazon to change their algorithms to make it more fair (more diverse recommendations)?
\subsubsection{Transparency}
Do users want transparency/explanations from Kiva/Amazon if they change their algorithms for fairness? do users want more transparency/explanations about fairness goals of a system whether or not an algorithm is changed? Transparency helps people detect the errors and biases and provides an opportunity of communication between a system and its users.
\subsubsection{Trust}
Which organization do users trust more and why? people trust a non-profit like Kiva more since the main goal is benevolent in the first place but it is different in for-profits since they are a business and their main goal is monetary. 
\subsubsection{Explanations}
Do users expect explanations? Does adding explanations increase trust in the system?



% \begin{figure}
%   \includegraphics[width=.9\columnwidth]{figures/ea-figure2}
%   \caption{If your figure has a light background, you can set its
%     outline to light gray, like this, to make a box around
%     it.}\label{fig:bats}
% \end{figure}

% \begin{marginfigure}[-35pc]
%   \begin{minipage}{\marginparwidth}
%     \centering
%     \includegraphics[width=0.9\marginparwidth]{figures/cats}
%     \caption{In this image, the cats are tessellated within a square
%       frame. Images should also have captions and be within the
%       boundaries of the sidebar on page~\pageref{sec:sidebar}. Photo:
%       \cczero~jofish on Flickr.}~\label{fig:marginfig}
%   \end{minipage}
% \end{marginfigure}

\section{Accessibility}
The Executive Council of SIGCHI has committed to making SIGCHI
conferences more inclusive for researchers, practitioners, and
educators with disabilities. As a part of this goal, the all authors
are expected to work on improving the accessibility of their
submissions. Specifically, we encourage authors to carry out the
following five steps:
\begin{itemize}\compresslist%
\item Add alternative text (figure description) to all figures
\item Mark table headings
\item Generate a tagged PDF
\item Verify the default language
\item Set the tab order to ``Use Document Structure''
\end{itemize}

For links to detailed instructions and resources, please see:
\url{http://chi2020.acm.org/authors/papers/guide-to-an-accessible-submission/}

Unfortunately good tools do not yet exist to create tagged PDF files
from Latex. \LaTeX\ users will need to carry out all of the above
steps in the PDF directly using Adobe Acrobat, after the PDF has been
generated.


% \begin{figure*}
%   \centering
%   \includegraphics[width=1.3\columnwidth]{figures/map}
%   \caption{In this image, the map maximizes use of space. You can make
%     figures as wide as you need, up to a maximum of the full width of
%     both columns. Note that \LaTeX\ tends to render large figures on a
%     dedicated page. Image: \ccbynd~ayman on Flickr.}~\label{fig:cats}
% \end{figure*}



% \marginpar{\vspace{-23pc}So long as you don't type outside the right
%   margin or bleed into the gutter, it's okay to put annotations over
%   here on the left, too; this annotation is near Hawaii. You'll have
%   to manually align the margin paragraphs to your \LaTeX\ floats using
%   the \texttt{{\textbackslash}vspace{}} command.}

% \begin{margintable}[1pc]
%   \begin{minipage}{\marginparwidth}
%     \centering
%     \begin{tabular}{r r l}
%       & {\small \textbf{First}}
%       & {\small \textbf{Location}} \\
%       \toprule
%       Child & 22.5 & Melbourne \\
%       Adult & 22.0 & Bogot\'a \\
%       \midrule
%       Gene & 22.0 & Palo Alto \\
%       John & 34.5 & Minneapolis \\
%       \bottomrule
%     \end{tabular}
%     \caption{A simple narrow table in the left margin
%       space.}~\label{tab:table2}
%   \end{minipage}
% \end{margintable}
\section{Discussion}
Maybe a discussion here about the results of the interviews? Or this would go in the Interview Analyses section...
\section{Conclusion / Closing Remarks / Future Work}
Something here to conclude
\section{Acknowledgements}
We thank all the volunteers, publications support, staff, and authors
who wrote and provided helpful comments on previous versions of this
document. As well authors 1, 2, and 3 gratefully acknowledge the grant
from NSF (\#1234--2222--ABC). Author 4 for example may want to
acknowledge a supervisor/manager from their original employer. This
whole paragraph is just for example. Some of the references cited in
this paper are included for illustrative purposes only.

\section{References Format}
Your references should be published materials accessible to the
public. Internal technical reports may be cited only if they are
easily accessible and may be obtained by any reader for a nominal
fee. Proprietary information may not be cited. Private communications
should be acknowledged in the main text, not referenced (e.g.,
[Golovchinsky, personal communication]). References must be the same
font size as other body text. References should be in alphabetical
order by last name of first author. Use a numbered list of references
at the end of the article, ordered alphabetically by last name of
first author, and referenced by numbers in brackets. For papers from
conference proceedings, include the title of the paper and the name of
the conference. Do not include the location of the conference or the
exact date; do include the page numbers if available. 

References should be in ACM citation format:
\url{http://www.acm.org/publications/submissions/latex_style}.  This
includes citations to Internet
resources~\cite{CHINOSAUR:venue,cavender:writing,psy:gangnam}
according to ACM format, although it is often appropriate to include
URLs directly in the text, as above. Example reference formatting for
individual journal articles~\cite{ethics}, articles in conference
proceedings~\cite{Klemmer:2002:WSC:503376.503378},
books~\cite{Schwartz:1995:GBF}, theses~\cite{sutherland:sketchpad},
book chapters~\cite{winner:politics}, an entire journal
issue~\cite{kaye:puc},
websites~\cite{acm_categories,cavender:writing},
tweets~\cite{CHINOSAUR:venue}, patents~\cite{heilig:sensorama}, 
games~\cite{supermetroid:snes}, and
online videos~\cite{psy:gangnam} is given here.  See the examples of
citations at the end of this document and in the accompanying
\texttt{BibTeX} document. This formatting is a edited version of the
format automatically generated by the ACM Digital Library
(\url{http://dl.acm.org}) as ``ACM Ref''. DOI and/or URL links are
optional but encouraged as are full first names. Note that the
Hyperlink style used throughout this document uses blue links;
however, URLs in the references section may optionally appear in
black.

\balance{}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:


==> toDoList.tex <==
— Combine the related work in the introduction section.
— Future Work : Talk about the issues that are going to the next paper.
Talk about the Kiva survey.
And some themes that did not make into this paper.


